Think Twice Before Trusting: Self-Detection for Large Language Models through Comprehensive Answer Reflection

Self-detection for Large Language Models (LLMs) seeks to evaluate the trustworthiness of the LLM's output by leveraging its own capabilities, thereby alleviating the issue of output hallucination. However, existing self-detection approaches only retrospectively evaluate answers generated by LLM, typically leading to the over-trust in incorrectly generated answers. To tackle this limitation, we propose a novel self-detection paradigm that considers the comprehensive answer space beyond LLM-generated answers. It thoroughly compares the trustworthiness of multiple candidate answers to mitigate the over-trust in LLM-generated incorrect answers. Building upon this paradigm, we introduce a two-step framework, which firstly instructs LLM to reflect and provide justifications for each candidate answer, and then aggregates the justifications for comprehensive target answer evaluation. This framework can be seamlessly integrated with existing approaches for superior self-detection. Extensive experiments on six datasets spanning three tasks demonstrate the effectiveness of the proposed framework.

==> sections/previous_intros/1_introduction_v1.tex <==
\section{Introduction}

% P1:
% 背景
% Large language models are one of the most powerful AI models nowadays. However, LLMs suffer from hallucination issue, and could generate erroneous outputs, which hinders the trustability. 
% One promising direction to improve trustability is confidence elicitation. 
% 过程
% For an output generated by LLM, we want to obtain the LLM confidence towards the answer. 
% 本质
% the confidence express LLM's uncertainty towards the answer, i.e., the reliability of answer regarding the input. 
% 例子
% This paper studies the black-box API LLMs such as ChatGPT and GPT-4. 
% A very common idea of confidence elicitation on black-box API LLMs is to sample multiple response and estimate the probability of the target answer. where answer with higher probability is more trustable. 
% 意义
% The target of confidence elicitation is calibration, confidence align with actual accuracy. In this way, the confidence can be used for identifying likely-wrong answers. 
% 问题。 
% however, LLM calibration is hard to achieve, often involves overconfidence issue (knowing, verbalized, cape). 
% This is because LLM cannot distinguish the correctness of the answers (self-correct), and thus getting overconfidence on the wrong samples.  

% For example, a common approach for black-box API LLM is sampling multiple outputs and use the estimated output probability as its confidence score. 

Large language models (LLM) are among the most potent AI models in today's landscape, where the state-of-the-art LLMs usually takes the form of black-box API. 
However, even the state-of-the-art LLMs are susceptible to hallucination and production of erroneous outputs, posing a significant challenge to their trustability. 
% 不是很能串起来。
A promising research direction for enhancing LLM trustability is confidence estimation. 
Given a question, we intend to obtain not only the LLM-generated answer, but also the LLM confidence level on the answer, representing LLM's certainty towards the accuracy of the answer. 
The goal of confidence estimation lies in achieving calibration, \ie ensuring that the confidence level align with actual answer accuracy, where the calibrated confidence scores could be useful for discerning and potentially rejecting unreliable answers. % , fostering more effective human-LLM collaboration. 
However, the problem lies in the difficulty of achieving calibration for LLM, often giving rise to the overconfidence issue. 
% what is the bias?
\textbf{The LLM may be inherent biased towards trusting its generated answers, resulting in difficulty to discern the incorrect answers and a tendency to assign overly high confidence scores to them. }
% 三个citation，三个证据。

% P2: 
% 总起
% to solve the problem and achieve better calibration. There are two lines of work. This paper mainly focuses on black-box API LLM, where the state-of-the-art models are usually in this form. 
% 起好名字。
% Firstly, Prompt ensemble. Using various instruction templates (), and changing the phrasing of the task input (). Aiming at removes the context bias between input and answer (), for better estimation of answer probability distribution. 
% Secondly, using alternative evaluation objectives. Instead of getting answer probability, they evaluate answer from other perspectives to know the reliability of A regarding input. such as token probability, self-verification, evaluate CoT, yet some are designed limited to certain domains.  
% 关键句。
% However, these two lines of research has a major limitation. 
% Because these confidence elicitation methods are targeted on a single LLM-predicted A (figure 1 b), or distribution for answers (figure 1 a), the LLM probably has intrinsic bias towards this A that it predicts, thus causing the overconfidence issue on this LLM-predicted A. 
% 到底对不对？

Prior research has attempted to addressed the overconfidence issue in LLMs to enhance calibration. 
Calibration methods within this domain can be broadly classified into two categories. 
The first category includes prompt ensemble methods that utilize various instruction templates and diverse rephrasing of the question to eliminate the context bias between the question and answer, enabling a more accurate estimation of the answer probability as the confidence score. 
The second category involves estimating the answer accuracy from various perspectives. Instead of eliciting the answer probability from LLM, these approaches utilize different evaluation objectives on LLM to estimate the answer accuracy, such as the probability of ``True" judgment, masked question verification, and evaluation on the CoT reasoning. 
% 这个方法的描述有问题。
% 需要定义bias, LLM 相信但是答案错了。正确的没事。
However, both lines of research share a significant limitation. 
\textbf{Because these methods merely target at the confidence estimation of a single LLM-generated answer, 
LLM may still be biased on the incorrect ones and be overconfident on them.} 




% P3: 
% We propose a new paradigm of confidence elicitation. 
% 起名字。
% Reflection on multiple candidate answers for better confidence calibration. 
% The new paradigm consists of two steps.
% Assume the input Q, and multiple candidate answers A, A', A''. 
% Step one is to scrutinize each I-A_i pair to evaluate the credibility of each A being I's output. 
% step two is to jointly consider the evaluation of multiple I A_o pairs for obtaining the confidence toward answer A. 
% 词需要打磨。
% 这么做的好处。
% By comprehensively evaluate and compare the credibility of candidate As, 
% the level of I A credibility can be more precicely judged. 
% therefore, the overconfidence on wrong A can be potentially mitigated. 
% 例子
% 
% CF实验。
% Our preliminary experiment demonstrates the effectiveness of considering multiple candidate Answer on calibration. (\cf section 2). 

% biased answer, target answer

Based on the limitation, we introduce a novel paradigm for confidence estimation on black-box API LLMs, \textbf{which involves jointly considering various candidate answers to enhance confidence calibration on the target answer}.
The first step involves scrutinizing each question-answer pair to assess the trustability of the answer as the correct answer to the question. % 冗余
Then, these assessment over various answers are jointly compared to derive a more precise confidence on the target answer. 
% 好处是什么？
By thoroughly thinking and comparing various candidate answers' trustability, the overconfidence on the biased answer can be mitigated when a candidate answer shows better trustability than the biased answer.  
% incorrect target answer == biased answer. 
% For example, in sentiment analysis, if the sentence is found to contain several positive words, the confidence of being negative should be reduced accordingly. 
Our preliminary experiments demonstrate the effectiveness of considering multiple answers in improving calibration. 


% P4:
% To achieve the proposed paradigm, there are several key considerations.
% Firstly, how to resist the intrinsic bias of LLM to precisely evaluate the credibility of I A', where A' is not the predicted answer of LLM. 
% Secondly, how to effectively aggregate the evaluation of multiple I A' pairs to elicit the calibrated confidence of A. 
% 
% 
% 
% 

Achieving the proposed paradigm requires addressing two key considerations. 
Firstly, how to overcome the inherent bias of LLM to accurately assess the trustability of each question-answer pair, particularly for the candidate answers that are not biased by LLM. 
% 冗余。
Secondly, how to effectively aggregate the assessment across multiple question-answer pairs to achieve effective confidence calibration on the target answer. 
These considerations have motivated us to propose the following framework. 

% P5:
% In this paper, we propose a novel framework to implement the proposed paradigm: Think Twice Before Trusting (T^3). 
% 一句话描述我们的framework在做什么。
% Our framework achieves calibrated confidence by reflecting on the trustability of each candidate IA pairs and jointly consider their trustability. 

% Specifically, we first instruct LLM to ``Think twice": try to generate explanation for the trustability on each IA pair. 
% Then, we utilize prompt-based method to incorporate all explanations into a more comprehensive confidence elicitation on A. 

% Extensive experiments on six datasets of three tasks shows improved calibration of T^3 over baselines from both previous paradigms. 
% Notably, T^3 can be combined with various existing techniques to further boost the calibration performance. 

% Our contribution are threefold. 
% firstly, we summarize the existing paradigms for confidence elicitation on black box API LLM, and propose a novel paradigm. 
% secondly, we propose a novel framework to implement which can be combines with existing methods.
% finally, we conduct extensive experiments, validating the rationality of the proposed paradigm and framework. 

In this paper, we introduce a novel framework for confidence calibration on black-box API LLMs, \underline{T}hink \underline{T}wice Before \underline{T}rusting ($T^3$).
\textbf{Our framework achieves calibrated confidence by 
adopting different viewpoints to explain the trustability for each question-answer pair 
before estimating the confidence of the target answer. }
Firstly, the LLM is instructed to consider each answer's viewpoint and endeavor to generate explanations regarding the potential correctness of each question-answer pair. % 不太对。
Subsequently, a prompt-based method is employed to integrate these explanations for joint consideration in the confidence estimation process for the target answer. 
Extensive experiments on six datasets across three tasks show improved calibration of $T^3$ compared to baselines from previous paradigms. 
Notably, $T^3$ can seamlessly integrate with existing methods, providing a versatile solution to further enhance calibration performance. 
Our contributions are three-fold. 
Firstly, we summarize the existing paradigms for confidence elicitation in black-box API LLMs, and introduce a novel paradigm to address their limitations. 
Secondly, we present a novel framework to achieve the proposed paradigm, which can be easily combined with existing methods. 
Finally, we conduct extensive experiments, validating the effectiveness of the proposed paradigm and framework. 





==> sections/previous_intros/1_introduction_v2.tex <==
\section{Introduction}

% P1

LLMs are among the most potent AI models in today's landscape, yet are vulnerable to hallucination \cite{zhang2023siren, li2023halueval} and the generation of erroneous outputs \cite{golovneva2022roscoe, bang2023multitask}, posing a significant challenge to the trustability of their outputs.
A promising research direction for improving LLM trustability is confidence estimation \cite{guo2017calibration, lin2022teaching}. 
Given a question, the objective is to obtain not only the LLM-generated answer, but also the LLM's confidence level representing the LLM's certainty on the accuracy of the answer. 
The aim of confidence estimation is to achieve calibration, ensuring that the confidence level aligns with actual answer accuracy, which could be valuable for distinguishing and rejecting unreliable answers \cite{kamath2020selective}. 
However, the challenge lies in the difficulty of achieving calibration for LLM, often leading to the overconfidence issue.  
The LLM may be inherently biased towards trusting its generated answers \cite{mielke2022reducing, ling2023deductive}, making it hard to truly discern incorrect answers \cite{huang2023large} and exhibiting a tendency to assign overly high confidence scores to them \cite{si2022prompting, xiong2023can}.


\begin{figure}[t]
    \centering
    \includegraphics[width = 0.5\textwidth]{figures/intro.pdf}
    \caption{An illustration of our TTA framework for calibrated confidence estimation. LLM is instructed to reflect on the trustability of each candidate answer before estimating its confidence on the target answer. }
    \vspace{-20pt}
    \label{fig:intro}
\end{figure}

% P2: 

Previous studies have attempted to tackle the overconfidence issue to improve calibration on black-box API LLM\footnote{Our research scope is black-box API LLM, as the state-of-the-art LLMs usually manifest as this form \cite{achiam2023gpt, chatgpt}}, which can be broadly summarized into two paradigms. 
The first paradigm includes prompt ensemble methods. They assume that overconfidence is partly due to the 
context bias between the question and answer, and employ various instruction templates and diverse rephrasing of the question to achieve better answer probability estimation as the confidence score \cite{jiang2023calibrating, zhao2023knowing}. 
The second paradigm focuses on LLM self-evaluation to estimate the answer accuracy, designing instructions such as asking LLM about the answer truthfulness \cite{kadavath2022language} or examining the Chain-of-Thought (CoT) reasoning \cite{miao2023selfcheck}. 
However, both lines of research share a significant limitation. 
Because these methods only consider confidence estimation on a single target answer generated by LLM, the LLM may still contain bias towards incorrect answer and be overconfident in them.



% P3:
% incorrect target answer == biased answer. 

Based on the limitation, we introduce a novel paradigm, which involves the consideration of multiple candidate answers to enhance confidence calibration. 
Firstly, the LLM scrutinizes a variety of question-answer pairs to assess the trustability of the answer as the correct response to the question. 
Subsequently, the assessment across different answers are aggregated to derive a better confidence score for the target answer. 
The overconfidence in the incorrect target answers can be alleviated when some candidate answers demonstrate better trustability. 
Our preliminary experiments reveal the effectiveness of considering multiple answers in reducing overconfidence (\cf Section~\ref{para:prelim_exp}). 



% P4:
Accomplishing the proposed paradigm necessitates addressing two key considerations.  
Firstly, there is the challenge of resisting the inherent bias of LLM to precisely evaluate the trustability of each question-answer pair. 
Secondly, there is the task of aggregating the assessments of multiple question-answer pairs in the confidence estimation of the target answer. 
These considerations have inspired us to present the following framework.


% P5: 
In this paper, we present a novel confidence estimation framework to tackle the overconfidence issue of LLMs, named \underline{T}hink \underline{T}wice before \underline{A}ssure (TTA). 
Our framework pushes LLM to reflect and justify from different answers' perspectives before confidence estimation on the target answer. 
Firstly, the LLM is instructed to generate explanations regarding the potential correctness of each answer. 
Subsequently, a prompt-based method is employed to integrate these explanations into joint confidence estimation for the target answer. 
Extensive experiments on six datasets across three tasks show improved calibration of TTA over methods from existing paradigms. 
Notably, TTA can be combined with existing methods to further improve calibration. 
Our contributions are three-fold. 
\begin{itemize}
    \item We categorize existing confidence estimation approaches for mitigating overconfidence issue in LLM into two paradigms, and introduce a novel paradigm to address their limitation.
    \item We present a novel TTA framework to improve calibration by reflecting on multiple answers' perspectives, which can be easily combined with existing methods. 
    \item We conduct extensive experiments on three NLP tasks, validating the rationality of and effectiveness of the proposed framework. 
\end{itemize}



==> sections/previous_intros/1_introduction_v3.tex <==
\section{Introduction}

% P1

LLM suffers from the hallucination issue \cite{zhang2023siren, li2023halueval, golovneva2022roscoe, bang2023multitask}, which poses a significant challenge to the trustability of its outputs. 
A promising research direction for evaluating the output trustability is confidence estimation \cite{guo2017calibration, lin2022teaching}, which could be useful for identifying and rejecting unreliable outputs \cite{kamath2020selective}. 
% We aim to study this technique on black-box API LLM \cite{achiam2023gpt, chatgpt}.
% In addition to generating an answer to the given question, confidence estimation aims to obtain LLM's confidence level representing the LLM's certainty on the accuracy of the answer. 
Given a question, confidence estimation aims to acquire LLM's confidence level on its generated answer, which reflects the LLM's certainty regarding the accuracy of the answer. 
The core of confidence estimation is to achieve calibration \cite{lin2022teaching}, ensuring that the confidence level aligns with the actual answer accuracy. 
% In this paper, we aim to enhance calibrated confidence estimation for black-box API LLMs due to their excellent performance and inherent challenges in confidence estimation \cite{achiam2023gpt, chatgpt}. 
In this paper, we aim to calibrate confidence estimation for black-box API LLMs due to their excellent performance \cite{achiam2023gpt, chatgpt}. 
% , as the state-of-the-art LLMs usually manifest in this form \cite{achiam2023gpt, chatgpt}.



\begin{figure}[]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{0cm}
    \centering
    \includegraphics[width = 0.5\textwidth]{figures/intro1.pdf}
    \caption{An illustration of our \textit{Think Twice before Assure} framework for mitigating LLM overconfidence. LLM is instructed to reflect on the trustability of each answer before joint confidence estimation. }
    \vspace{-15pt}
    \label{fig:intro}
\end{figure}


% \footnote{Our research scope is black-box API LLM, as the state-of-the-art LLMs usually manifest as this form \cite{achiam2023gpt, chatgpt}}, which can be broadly summarized into two paradigms. 

% P2: 
The key to achieving calibrated confidence estimation for black-box LLM lies in addressing the overconfidence issue. 
The LLM may be inherently biased towards trusting its generated answers \cite{mielke2022reducing, ling2023deductive}, making it hard to truly discern incorrect answers \cite{huang2023large} and exhibiting a tendency to assign overly high confidence scores to them \cite{si2022prompting, xiong2023can}. 
Previous studies attempting to tackle the overconfidence issue can be broadly categorized into two paradigms. 
The first paradigm mainly assumes that overconfidence is partly caused by the context bias between the prompt and the answer and thus performs prompt ensemble by constructing various instruction templates and diverse rephrasing of the question 
%to achieve better answer probability estimation as the confidence score 
\cite{jiang2023calibrating, zhao2023knowing}. 
% , based on their assumption that overconfidence is partly due to the context bias between the question and the answer. 
The second paradigm focuses on LLM self-evaluation, designing instructions such as asking LLM about the answer truthfulness \cite{kadavath2022language} or examining the Chain-of-Thought (CoT) reasoning \cite{miao2023selfcheck}. 
However, both lines of research only consider a single target answer generated by LLM, and the LLM may still contain bias towards the incorrect answers and be overconfident in them.


% P3:
% incorrect target answer == biased answer. 

To tackle this limitation, we introduce a new multi-answer evaluation paradigm involving the consideration of multiple candidate answers to enhance confidence calibration (\cf Figure~\ref{fig:paradigms}), where the evaluation of potentially correct answers helps to reduce the biased trust in the incorrect ones. 
This paradigm scrutinizes various answers on the trustability of being the correct response to the question, and aggregates these evaluations to derive a better confidence score for the target answer. 
The biased trust in the incorrect target answers can be alleviated through the trustability comparison with other more trustable answers.
%Firstly, the LLM scrutinizes various question-answer pairs to assess the trustability of each answer as the correct response to the question. 
%Subsequently, the assessment across different answers is aggregated to derive a better confidence score for the target answer. 
% The overconfidence in the incorrect target answers can be alleviated when some candidate answers demonstrate better trustability. 
Our preliminary experiments reveal the efficacy of considering multiple answers to reduce overconfidence (\cf Section~\ref{para:prelim_exp}). 
% 如果这一段只high level介绍paradigm，下一段仔细介绍，可以吗？
% 没提到correct answer 有问题吗？




% P4:
There are two key considerations in arriving at the proposed paradigm: resisting the inherent bias of LLM to precisely evaluate the trustability of each question-answer pair, and aggregating these assessments in the confidence estimation of the target answer. 
In this light, we present a novel confidence estimation framework to tackle the overconfidence issue of LLMs, named \underline{T}hink \underline{T}wice before \underline{A}ssure (TTA) (\cf Figure~\ref{fig:intro}). 
Our framework pushes LLM to reflect and justify from different answers' perspectives before confidence estimation on the target answer. 
Firstly, the LLM is instructed to generate justifications regarding the potential correctness of each answer. 
Subsequently, a prompt-based method is employed to integrate these justifications into joint confidence estimation for the target answer. 
Extensive experiments on six datasets across three tasks show improved calibration of TTA over methods from existing paradigms. 
Notably, TTA can be combined with other methods to further improve calibration. 
Our contributions are three-fold. 
\begin{itemize}[leftmargin=*]
    \item We introduce a novel confidence estimation paradigm for mitigating the overconfidence issue in LLM, addressing the limitation of existing paradigms by reflection on multiple answers. 
    \item We present a novel TTA framework to implement the multi-answer evaluation paradigm, which can be easily combined with existing methods. 
    \item We conduct extensive experiments on three NLP tasks with six datasets, validating the rationality and effectiveness of the proposed framework. 
\end{itemize}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 0.5\textwidth]{figures/paradigms.pdf}
%     \caption{Two existing paradigms to tackle the overconfidence issue for LLM and our proposed paradigm. }
%     \label{fig:paradigms}
% \end{figure}


% 两种模式，问题不太大，一种是confidence,probability，一种是detection, 代表性的是P(true)。需要highlight他们的区别。
% limitation的描述很不好，根本原因不是只考虑了一个答案，而是只考虑了LLM生成的答案，需要一些其他非正确答案来辅助。
% 需要描述出两个目标，ECE for calibration 和 AUROC for detection。 
% 两个目标问题。
% 展示overconfidence需要画calibration的图。

% figure 3 画成roc曲线的对比。
% related work 写成confidence estimation和 self-evaluation/detection. 
% 实验放ECE问题不大。考虑换成auroc图。

==> sections/previous_intros/2_related_work.tex <==
\section{Related Work}


\paragraph{Confidence Elicitation for LLM.}
The idea of confidence elicitation originated from uncertainty estimation. 
In the era of LLM, some still requires token probability, not suitable for us. (SE. look before your leap, maxent, shifting attn, )
how can we know when LLM know \cite{jiang2021can}. 
long horizon temperature scaling \cite{shih2023long}. 
% unimportant, just a few. 

Closer to us, require no token prob, suitable for bb llm. 
many estimate probability. 
self-cons. to estimate distribution. 
top-K verbalized. verbalized. for distribution. 
in NLG, ranking. 
generating with confidence. NLG, no overconf, ranking outputs. 

% train small model, gpt-4. 
orthogonal. 
Using trained model to judge: GPT-4 oracle. Gather training data. trained model.
pareto optimal. 
lin. teaching 
Using external tools: 1 or 2. 

\paragraph{The Overconfidence Issue and Solutions.}
where exist: 
1) verbalized can llm. clearly overconf. 
2) selfcheck: maj is not best. 
LLM is shown to be intrinsically tend to believe in its prediction. 
mielke. (not bb). 
and cannot clearly tell the wrong ones from correct ones. 
3) deductive verification. cannot check all steps at once. LLM cannot do self-correct reasoning yet. 



where tackle:

The first category: ensemble method. 
knowing, SAC3 para.
cape, Ren Jie. ensemble instruction, position bias.
self-contrast. Self-Contrast: Better Reflection Through Inconsistent Solving Perspectives. perspectives. have idea. 

The second category: 
Self-evaluation methods. 
P(True): token probability
selfcheck: 
DV: 
selfcheckgpt: 
self-verification, GPT-4-code
hallucinating reference \cite{agrawal2023language}. 
some are limited in certain domains. 

A mix of several methods from different cate (BSDETECTOR, Hybrid)

\paragraph{Application of LLM Confidence.}
% The use of confidence. 
The LLM confidence is used in many ways. 
1. fix generation hallucination error. with cons. 
2. Yuxi: guide CoT decoding. 
3. decomposing. find out ambig question. 
4. selective prediction. 
See liangming survey. 






==> sections/previous_intros/3_task_formulation.tex <==
\section{Problem Formulation}


\paragraph{Confidence Estimation for LLM.}
% The task of confidence estimation for LLM can be illustrated as follow. 
We formulate the task of confidence estimation for LLM as follows. 
% LLM receives the input of the given question $q$ combined with the prompt $p$, which consists of an instruction and optional in-context examples, to generate the answer $a$. 
Given the input comprising of question $q$ combined with prompt $p$, which consists of an instruction and optional in-context examples, LLM can generate the answer $a$~\cite{brown2020language}, denoted as the target answer. 
% We intend to obtain the LLM confidence level on $a$, in the form of a confidence score $c \in \mathcal{R}$. 
Thereafter, confidence estimation aims to obtain the LLM's confidence level on $a$, in the form of a confidence score $c \in \mathcal{R}$.  
Denoting the confidence estimation strategy as a function $CE(\cdot)$, this process can be abstracted as 
\begin{align}
    \label{eq:llm_prediction}
    a & = LLM(p(q)),\\
    c & = CE(LLM(\cdot), p(q), a).
\end{align}
A common idea of $CE(\cdot)$ is to utilize the LLM output probability of $a$ to estimate the confidence score \cite{kuhn2023semantic, hu2023uncertainty}, denoted as $c = Pr(LLM(\cdot), p(q), a)$. 
% For black-box API LLM where the token probability is unavailable, this can be achieved by self-consistency \cite{wang2022self, si2022prompting, lin2023generating}
% , \ie estimating the probability of $a$ by sampling $N > 1$ responses from LLM (\eg nucleus sampling \cite{Holtzman2020The}), % Assume that $N$ responses are sampled, we have 
% and verbalized method \cite{lin2022teaching, tian2023just}, \ie prompting LLM to output the $K$ most likely answers and their corresponding probabilities in one response (denote the prompt as $p^t$). 
% \begin{align}
%     & c = Pr(LLM(\cdot), p(q), a) \\\notag
%     \text{e.g.,}& \text{self-consistency,} \\    \label{eq:self-cons}
%     & c = \frac{\sum_{i=1}^N \mathbb{1} (a_i = a)}{N} \\ \notag
%     &\text{where }  a_1, a_2, ..., a_N = LLM(p(q)) \\\notag
%     \text{e.g.,}&\text{Top-K verbalized,} \\ \label{eq:verb}
%     & a_1, c_1, ... a_K, c_K = LLM(p^t(q)) \\ \notag
%     & c = c_k, \text{where }a_k = a, k \in 1, ..., K
% \end{align}
For black-box API LLM where the token probability is unavailable, this can be achieved by self-consistency \cite{wang2022self, si2022prompting, lin2023generating} and verbalized methods \cite{lin2022teaching, tian2023just}. 
Self-consistency methods estimate the probability of answer $a$ by sampling $D > 1$ responses from LLM (\eg using nucleus sampling \cite{Holtzman2020The}). Formally, we have
\begin{align}
    \label{eq:self-cons}
    & c = \frac{\sum_{i=1}^D \mathbb{1} (a_i = a)}{D}, \\ \notag
    % &\text{where }  a_1, a_2, ..., a_N = LLM(p(q)). \notag
    &\text{where }  a_i = LLM(p(q)). \notag
\end{align}
Besides, the verbalized methods leverage a well-designed prompt $p^b$ to instruct the LLM to output the $K$ most likely answers and their corresponding probabilities in one response, \ie 
\begin{align}
    \label{eq:verb}
    & [\{a_1, c_1\}, ... \{a_K, c_K\}] = LLM(p^b(q)). 
\end{align}
where $[\cdot]$ denotes the concatenation of the $K$ most likely answers with their probabilities. 
% \begin{align}
%     \label{eq:verb}
%     & a_1, c_1, ... a_K, c_K = LLM(p^t(q)), \\ \notag
%     & c = c_k, \text{where }a_k = a, k \in 1, ..., K. 
% \end{align}

% \fb{Note: need to add the description about Pr, N and L }
% added

% \begin{align}
%     a_1, a_2, ..., a_N = LLM(p(q)) \\ \label{eq:self-cons}
%     c = \frac{\sum_{i=1}^N \mathbb{1} (a_i = a)}{N} 
% \end{align}

% 第二个公式改得更general更好。

% The verbalized method utilize a special prompt $p^v$ to instruct LLM to output the predicted answers along with their confidence scores in one response (See Appendix for prompts). 

% \begin{align}
%     a_1, c_1, ... a_N, c_N = LLM(p^v, q) \\
%     c = c_k, \text{where }a_k = a, k \in 1, ..., N
% \end{align}

% We summarize their idea as deriving the LLM probability of $a$
% \begin{align}
%     c = Pr(LLM(\cdot), p, q, a)
% \end{align}




% overconfidence 问题说明。
\paragraph{Overconfidence Issue and Existing Solution Paradigms.}
However, LLMs are prone to be overconfident. Both self-consistency and verbalized methods have a severe overconfidence issue, where they exhibit high confidence in some incorrect answers \cite{si2022prompting, xiong2023can}. 
% A major calibration issue of the self-consistency method stems from high confidence in incorrect answers, as observed by \citet{si2022prompting}, where the LLMs often repeat the incorrect answers in multiple sampled responses \cite{miao2023selfcheck}. 
%\citet{si2022prompting} observed that LLMs often repeat the incorrect answers in multiple sampled responses.% \cite{miao2023selfcheck}. 
% Moreover, the naive verbalized method ($K=1$) also shows significant overconfidence \cite{xiong2023can}. 
% Other confidence estimation methods, such as the verbalized method \cite{lin2022teaching}, also exhibit significant overconfidence \cite{xiong2023can}. 
In fact, LLM has a bias to blindly trust its generated answers, leading to difficulties in distinguishing the answer correctness \cite{huang2023large, ling2023deductive, mielke2022reducing, ren2023investigating}. 
%In fact, LLM struggles to distinguish the correctness of its generated answers, leading to a bias to blindly trust on them \cite{huang2023large, ling2023deductive, mielke2022reducing, ren2023investigating}.
% 定义bias是什么。
% 所以，对和错都很相信。导致score是一样的。
% Therefore, the overlapping of confidence scores between correct and incorrect answers poses a miscalibration challenge. 
As a result, it causes a miscalibration between the confidence score and the answer accuracy. 


We conclude the existing research addressing the overconfidence issue into two paradigms (\cf Figure~\ref{fig:paradigms}). 
The first paradigm includes prompt ensemble methods. 
% 承接前文的问题；
They posit that the overconfidence of LLM in $a$ is influenced by the context bias between $q$ and $a$ \cite{zhao2023knowing} or $p$ and $a$ \cite{jiang2023calibrating}. 
Therefore, they adopt different prompts, $\mathcal{P} = \{p_1, ..., p_M\}$, or various rephrasings of $q$, $\mathcal{Q}' = \{q'_1, ..., q'_M\}$, to alleviate the biased probability estimation of $a$. Assuming using $M$ different inputs, the first paradigm estimates the confidence $c$ by
\begin{align}
    &c = \frac{1}{M} \sum_{i=1}^M Pr(LLM(\cdot), p_i(q'_i), a), \\ \notag
    &\text{where } p_i \in \mathcal{P}, q'_i \in \mathcal{Q}'.  
\end{align}

% 后面有没有k?

\begin{figure}[t]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{0cm}
    \centering
    \includegraphics[width = 0.47\textwidth]{figures/paradigms.pdf}
    \caption{Two existing paradigms to tackle the overconfidence issue for LLM and our proposed multi-answer evaluation paradigm. }
    \vspace{-10pt}
    \label{fig:paradigms}
\end{figure}

% The second paradigm involves the self-evaluation method, where researchers design instructions to guide LLM in self-evaluating the correctness of $a$ from different perspectives, denoted as $Co(\cdot)$. 
The second paradigm involves self-evaluation, which utilizes instructions to guide LLM in self-evaluating the correctness of $a$ from different perspectives, and uses the self-evaluated correctness as the confidence score, denoted as $Co(\cdot)$. Formally, 
\begin{align}
    c = Co(LLM(\cdot), p^t(q), a) \label{eq:ptrue}.
\end{align}
where $p^t$ denotes the evaluation prompt. 
This includes assessing the correctness of the CoT reasoning of $a$ \cite{miao2023selfcheck}, completing masked questions using $a$ \cite{weng-etal-2023-large}, and checking input-output consistency \cite{manakul-etal-2023-selfcheckgpt}. 
% For example, it has been found that estimating the word probability of asking whether $a$ is the ``True" answer to $q$ is better calibrated than estimating the answer probability \cite{kadavath2022language}, denoted as P(True), $c = Pr(LLM(\cdot), p^t(q, a), \text{\textit{True}})$, (see Appendix~\ref{sec:appe_prompts} for $p^t$).
To give an example, the P(True) method \cite{kadavath2022language} asks LLM whether $a$ is the true answer to $q$ via the prompt $p^r$, and uses the probability of ``True'' in the sampled LLM responses as the confidence score, $c = Pr(LLM(\cdot), p^r(q, a), \text{\textit{True}})$. 
% as illustrated below, 
% \begin{align}
%     \label{eq:ptrue}
%     % c &= Co(LLM(\cdot), p^t(q), a) \\ \notag
%      c = Pr(LLM(\cdot), p^t(q, a), \text{\textit{True}}) 
% \end{align}
% \fb{removed the $t$ in $p^t$ }
% added t in Co
% where $p^t$ denotes the prompt asking whether $a$ is the true answer of $q$ (see Appendix~\ref{sec:appe_prompts} for details).
The two paradigms can also be combined for better calibration \cite{xiong2023can, chen2023quantifying, ren2023self, agrawal2023language}. 

\paragraph{A New Multi-Answer Evaluation Paradigm. }
% bias是什么?
A notable limitation of the existing two paradigms is that they merely focus on confidence estimation for a single LLM-generated answer $a$, in which LLM may be overconfident. 
Despite efforts in context bias elimination and self-evaluation, LLM's biased trust in the incorrect $a$ may persist. 
% However, we think that this could be mitigated if LLM had thoroughly compared the trustability of more candidate answers of $q$. 
However, we think that this biased trust could be alleviated if LLM had thoroughly compared the trustability of more candidate answers of $q$. 
If other answers had a strong tendency to be correct, the high confidence in $a$ could be diminished, reducing the overconfidence risk. 
% 只能降低conf，因为存在bias，不太可能把第一名比下去。
Therefore, we propose a novel multi-answer evaluation paradigm that considers $N$ potential answers, denoted as $\{a^q_1, a^q_2, ..., a^q_N\}$ in confidence estimation\footnote{In the case of multiple-choice questions, candidate answers are naturally provided. 
% However, for questions without predefined choices, it is suggested to prompt the LLM to generate outputs that can serve as choices \cite{jiang2023calibrating}.
However, for questions without predefined choices, we can prompt the LLM to generate high-probability answers as candidates \cite{jiang2023calibrating}.}. 
First, LLM evaluates the trustability of each $q, a^q_i$ pair using a designated prompt $p^e$.
Then, all obtained evaluations $e_1,...,e_N$ are aggregated to derive a more refined confidence score for $a$, using the prompt $p^v$.
% Then, the obtained evaluations $e_1... e_n$ for all candidate answers are aggregated and compared across all candidate answers to derive a more calibrated confidence score for $a$, with the prompt $p^v$
% \fb{First, the initial evaluation $e_i$ of each pair ($q, a^q_i$), whose value is True or False, is obtained by using a designated prompt $p^e$. Then, all obtained evaluations $e_1... e_n$ are aggregated with the answer to derive a more refined confidence score for $a$ with the prompt $p^v$.}
\begin{align}
     \label{eq:gen_expl} 
     &c = Pr(LLM(\cdot), p^v(q, [e_1, ..., e_N]), a), \\
     \notag
     &\text{where } e_i = LLM(p^e(q, a^q_i)), i \in \{1, ..., N\}.
\end{align}
% where $[\cdot]$ denotes concatenation. 之前说过了。
This paradigm can also be combined with existing paradigms for better calibration (\cf Section~\ref{sec:main_results}). 

\paragraph{Preliminary Experiments.} \label{para:prelim_exp}

\begin{figure}
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \setlength{\belowcaptionskip}{0cm}
    \includegraphics[width = 0.5\textwidth]{figures/prelim_cf.pdf}
    \caption{Comparison of confidence estimation methods on CAD. \textit{w/ cf} denotes our strategy with counterfactual data. The AUROC is shown in the x-axis. The boxes on the left and right represent the confidence scores of incorrect and correct answers, respectively. }
    \vspace{-8pt}
    \label{fig:prelim_cf}
\end{figure}


We conduct a preliminary experiment to validate that considering more answers to adjust confidence scores is beneficial for calibration. 
Our hypothesis is that the confidence levels of other answers can be leveraged to identify and mitigate overconfidence in the incorrect $a$. 
%To demonstrate this, we employ an approximated setting using counterfactual question $\bar{q}$ with a different label from $q$, and utilize the contradiction between their predictions to identify potentially incorrect $a$. 
To demonstrate this, 
% instead of obtaining the confidence level of other answers on $q$ directly, 
% we employ an approximated setting by using counterfactual question $\bar{q}$ 
we employ counterfactual questions with different labels. 
Counterfactual question $\bar{q}$ is minimally edited from $q$ to have a different label with $q$. 
We aim to utilize the difference in $q$ and $\bar{q}$'s labels to identify unreliable LLM answers and adjust the confidence.  
Suppose the LLM-generated answers for $\bar{q}$ and $q$ are $\bar{a}$ and $a$, respectively. 
% Since $\bar{q}$ and $q$ have different labels, if $\bar{a}$ equals $a$, it shows that $a$ and $\bar{a}$ contains at least one wrong answer, thus the confidence of $a$ should be reduced according to the confidence of $\bar{a}$. 
If $\bar{a}$ equals $a$, $a$ and $\bar{a}$ must have at least one wrong answer since $\bar{q}$ and $q$ have different labels. Thus the confidence of $a$ should be reduced according to the confidence of $\bar{a}$ because the increasing confidence of $\bar{a}$ indicates the weakened confidence of $a$. 
Conversely, if $\bar{a}$ differs from $a$, $a$ and $\bar{a}$ are relatively trustable, and the confidence of $a$ can be an average of itself and $\bar{a}$'s confidence.  
Denoting the confidences of $a$ on $p(q)$ and $\bar{a}$ on $p(\bar{q})$ as $c_a$ and $c_{\bar{a}}$, respectively, the confidence of $a$ on $p(q)$ is re-calculated as
% We aim to utilize the contradiction of $q$ and $\bar{q}$'s predictions, denoted as $a$ and $\bar{a}$, to identify potentially incorrect $a$. 
% Suppose $\bar{q}$ has the prediction $\bar{a}$. If $\bar{a}$ equals $a$, $a$ is likely incorrect, and its confidence should be reduced based on the confidence level of $\bar{a}$. 
% Conversely, if $\bar{a}$ differs from $a$, $a$ is deemed trustworthy according to $\bar{a}$, and the confidence of $a$ should be an average of both questions. 
% Denoting the confidences of $a$ and $\bar{a}$ as $c_a$ and $c_{\bar{a}}$, respectively, 
\begin{align}
    c = 
    \begin{cases}
      \frac{1}{2} (c_a + c_{\bar{a}} )  & \text{if $a \neq \bar{a}$}, \\
      \frac{1}{2} (c_a + O(c_{\bar{a}}) )  & \text{else}.
    \end{cases}       
\end{align}
where $O(c_{\bar{a}})$ denotes the confidence that $\bar{q}$'s label is not $\bar{a}$. In a $k$-classification task, we roughly estimate $O(c_{\bar{a}}) = \frac{1}{k-1}(1 - c_{\bar{a}})$. 

We experiment with the CAD dataset \cite{kaushik2019learning}, which contains human-annotated original and counterfactual data pairs for sentiment analysis (SA) and natural language inference (NLI) tasks.
We compare the AUROC with self-consistency and Top-$K$ verbalized methods to evaluate the confidence calibration of LLM (see Section~\ref{sec:compared_methods} and Appendix~\ref{sec:appe_prelim_exp} for more details).  
Figure~\ref{fig:prelim_cf} shows the performance and the statistics of confidence scores for correct and incorrect answers, from which we can observe that 
1) the self-consistency and Top-$K$ verbalized methods have notable overconfidence. The incorrect answers have similar confidence scores as correct answers, making it challenging to distinguish them. 
2) Our strategy, denoted as \textit{w/ cf}, improves AUROC by lowering confidence scores on incorrect answers, showing that considering more answers has the potential to alleviate the overconfidence issue in incorrect answers. 
However, human-annotated counterfactual data is not easily available, motivating us to propose the following framework. 







